Computing the Cut Locus of a Riemannian Manifold via Optimal Transport

In this paper, we give a new characterization of the cut locus of a point on a compact Riemannian manifold as the zero set of the optimal transport density solution of the Monge-Kantorovich equations, a PDE formulation of the optimal transport problem with cost equal to the geodesic distance. Combining this result with an optimal transport numerical solver based on the so-called dynamical Monge-Kantorovich approach, we propose a novel framework for the numerical approximation of the cut locus of a point in a manifold. We show the applicability of the proposed method on a few examples settled on 2d-surfaces embedded in $R^{3}$ and discuss advantages and limitations.

==> myclasses.tex <==
%  35,% -> Partial differential equations \\
%  35J,% Partial differential equations of elliptic type \\
35J70\sep% Elliptic partial differential equations of degenerate type\\
49K20\sep % Problems involving partial differential equations \\
%  49M,%  Numerical Methods \\
49M25\sep%  Discrete approximations \\
49Q20\sep  %	Variational problems in a geometric measure-theoretic setting
58J05\sep % Elliptic equations on manifolds, general theory
%  65,% -> Numerical analysis \\
%  65N,% Partial differential equations, boundary value problems \\
65K10\sep   % Numerical optimization and variational techniques
65N30 % Finite elements, Rayleigh-Ritz and Galerkin methods, finite methods

